Price of Anarchy for Auction Revenue

This paper develops tools for welfare and revenue analyses of Bayes-Nash equilibria in asymmetric auctions with single-dimensional agents. We employ these tools to derive price of anarchy results for social welfare and revenue. Our approach separates the standard smoothness framework into two distinct parts, isolating the analysis common to any auction from the analysis specific to a given auction. The first part relates a bidder's contribution to welfare in equilibrium to their contribution to welfare in the optimal auction using the price the bidder faces for additional allocation. Intuitively, either an agent's utility and hence contribution to welfare is high, or the price she has to pay for additional allocation is high relative to her value. We call this condition value covering; it holds in every Bayes-Nash equilibrium of any auction. The second part, revenue covering, relates the prices bidders face for additional allocation to the revenue of the auction, using an auction's rules and feasibility constraints. Combining the two parts gives approximation results to the optimal welfare, and, under the right conditions, the optimal revenue. In mechanisms with reserve prices, our welfare results show approximation with respect to the optimal mechanism with the same reserves. As a center-piece result, we analyze the single-item first-price auction with individual monopoly reserves. When each distribution satisfies a regularity condition the auction's revenue is at least a $2e/(e-1) \approx 3.16$ approximation to the revenue of the optimal auction. We also give bounds for matroid auctions with first-price or all-pay semantics, and the generalized first-price position auction. Finally, we give an extension theorem for simultaneous composition, i.e., when multiple auctions are run simultaneously, with single-valued, unit-demand agents.

==> beyondpayyourbid_combinatorial.tex <==
\subsection{Combinatorial Winner-Pays-Bid Auctions}
\label{sec:fpacombinatorial}

We now consider the \emph{single-minded combinatorial auction} setting. We analyze two different winner-pays-bid mechanisms: one which allocates to the set of bidders with the highest total bid, and one which allocates greedily. The former mechanism can fall short of optimal by a factor of $\numitems$, the number of items. It is known from \cite{BL10}, though, that the latter mechanism is $\Theta(\sqrt{\numitems})$-approximation to the optimal welfare. We frame these two results in terms of revenue covering - the former mechanism is not $\revpar$-revenue covered for any $\revpar<\numitems$, whereas the greedy mechanism is $\sqrt{\numitems}$-revenue covered. (As a corollary, the revenue of the greedy mechanism with monopoly reserves is within a factor of $(\sqrt{\numitems}+1)\tfrac{e}{e-1}$ of optimal, when bidders have regular distributions.) This comparative analysis suggests the power of revenue covering as a design objective.\footnote{Subsequent to this work, \citet{DK15} showed that there is no winner-pays-bid mechanism for the single-minded combinatorial auction environment with a revenue covering parameter which is $o(\sqrt m)$.}

\paragraph{Single-Minded Combinatorial Auctions}
In a single-minded combinatorial auction feasibility environment, there are $\numitems$ indivisible items. Each bidder $\agent$ wishes to acquire a set of items $\wantsagent$ - she receives value $\valagent$ for receiving any superset of $\wantsagent$, and value 0 otherwise. An allocation vector $\alloc\in\{0,1\}^n$ is feasible if and only if it is possible to simultaneously allocate $\wantsagent$ to each $\agent$ with $\allocagent=1$.

\paragraph{Highest-Bids-Win Mechanism}
We first show that the optimal allocation algorithm in the absence of incentives performs poorly in equilibrium with winner-pays-bid semantics. Formally:

\begin{lemma}
\label{lem:combbad}
There exists a single-minded combinatorial auction environment where the highest-bids-win mechanism is not $\revpar$-revenue covered for any $\revpar<\numitems$.
\end{lemma}

\begin{proof}
Consider a setting with $\numitems$ items and $\numitems+2$ bidders. The first $\numitems$ bidders each want a single item - bidder $\mitem$ wants item $\mitem$, each with a value for allocation of 1, deterministically. The final two bidders, meanwhile, each want the grand bundle of all $\numitems$ items, with values of $1+\epsilon$, again deterministically. With appropriate tiebreaking, it is a BNE for each of the first $m$ agents to bid 0, while the final two bidders bid $1+\epsilon$. The optimal social welfare and revenue are both attained by selling to the first $\numitems$ bidders, for welfare and revenue of $\numitems$, yielding a price of anarchy of $\numitems$ for both welfare and revenue.

This equilibrium also lower bounds the revenue-covering parameter for the highest-bids-win mechanism. First, note that the total revenue of the mechanism is $1+\epsilon$. Next, consider the feasible allocation $\allocalt$ which allocates the first $\numitems$ bidders. For these bidders, they must bid at least $1+\epsilon$ to get allocated, at which point they get allocated with probability 1. It follows that for such bidders, $\expthresholdagent=1+\epsilon$, and hence $\sum_\agent \expthresholdagent\allocaltagent=(1+\epsilon)\numitems$, $\numitems$ times the mechanism's revenue.
\end{proof}



\paragraph{Greedy Allocation Mechanism} The \emph{greedy allocation mechanism} sorts bidders in non-increasing order of  $\actionagent/\sqrt{|\wantsagent|}$, where $\actionagent$ is the bid of agent $\agent$. In this order, it then adds bidders to the winning set whenever doing so would maintain feasibility. The greedy allocation rule is suboptimal in the absence of incentives. With winner-pays-bid semantics, however, it is $\sqrt{\numitems}$-revenue covered. In other words, the greedy rule possesses better incentive properties than highest-bids-win. This reproves the welfare result of \cite{LB09}. Moreover, a revenue result (with monopoly reserves and regular bidders) follows as a corollary.

The proof proceeds in three steps. First, we note a result of \cite{LOS02}: absent any inefficiency caused from incentives, the greedy allocation rule only loses a factor of $\sqrt{\numitems}$ compared to the highest-bids-win rule. Formally:
\begin{lemma}[\citealp{LOS02}]
\label{lem:greedyapx}
Let $\bidalloc(\actions)$ be the allocation selected by the greedy allocation rule under bid profile $\actions$, and $\allocalt$ be any other feasible allocation. Then
\begin{equation}
\sum\nolimits_\agent \actionagent\bidallocagent(\actions)\geq\sqrt{\numitems}\sum\nolimits_\agent\actionagent\allocalt.
\notag
\end{equation}
\end{lemma}

Next, we note that the greedy allocation rule lacks the pathology that ruined the welfare under highest-bids-win in the proof of Lemma~\ref{lem:combbad}. In the example, the high bids of the $(\numitems+1)$st and $(\numitems+2)$nd bidders discouraged participation from the other bidders - individually, each bidder would have needed to bid $1+\epsilon$ to win. As a group, though, the losing bidders could have won by increasing each of their bids by a tiny amount. The greedy allocation rule lacks this problem. We may increase the bids of every losing agent to their threshold without changing the outcome of a greedy mechanism. Formally:

\begin{lemma}
\label{lem:bossy}
Let $\actions$ be a profile of bids, let $\thresholdagent(\actionothers)$ be the critical price of bidder $\agent$ under the greedy allocation rule, and let $\bidalloc(\actions)$ be the corresponding allocation function. Further let $\actionsalt$ be any profile of bids such that if $\bidallocagent(\actions)=1$, then $\actionaltagent=\stratagent$, and if $\bidallocagent(\actions)=0$, then $\actionaltagent\leq \thresholdagent(\actionothers)$. Then $\bidalloc(\actions)=\bidalloc(\actionsalt)$.
\end{lemma}

\begin{proof}
Imagine changing $\actions$ to $\actionsalt$ by increasing one loser's bid at a time. Each time we increase a bid, say, of bidder $\agent$, two things remain true: (1) $\agent$ still loses - as long as $\actionaltagent\leq\thresholdagent(\actionothers)$, $\agent$ is after some other winning agent in the ordering, who wins some item in $\wantsagent$. (2) the threshold of every other losing agent $\agentalt$ remains unchanged - $\agentalt$ still wins if and only if $a_{\agent'}$ high enough to precede in the ordering all winners who get items in their set, which is not affected by $\agent$'s bid as long as $\agent$ still loses.
\end{proof}

Finally, we note that these two properties are enough to guarantee $\sqrt{\numitems}$-revenue covering.

\begin{lemma}
The winner-pays-bid greedy combinatorial auction is $\sqrt{\numitems}$-revenue covered.
\end{lemma}
\begin{proof}
We argue that for any action profile $\actions$ and alternate allocation $\allocalt$,
\begin{equation}
\sum\nolimits_\agent \actionagent\bidallocagent(\actions) \geq \tfrac{1}{\sqrt{\numitems}}\sum\nolimits_\agent \threshpt{\actionothers}\allocaltagent.
\notag
\end{equation}
Taking the expectation of both sides yields the desired inequality.

Let $\actionsalt$ be a vector of bids where losers under $\actions$ bid $\threshpt{\actionothers}$, while winners bid as before. The following inequalities hold, with justifications after.
\begin{align*}
\sum\nolimits_\agent \actionagent\bidallocagent(\actionothers) &= \sum\nolimits_\agent \actionaltagent\bidallocagent(\actionothers)&\\
&= \sum\nolimits_\agent \actionaltagent\bidallocagent(\actionsalt)\\
&\geq\tfrac{1}{\sqrt{\numitems}}\sum\nolimits_\agent\actionaltagent\allocaltagent\\
&\geq\tfrac{1}{\sqrt{\numitems}}\sum\nolimits_\agent \threshpt{\actionothers}\allocaltagent.
\end{align*}
The first line holds because $\actionsalt$ differs from $\actions$ only on the bids of losing agents. The second follows from Lemma~\ref{lem:bossy}, and the third from Lemma~\ref{lem:greedyapx}. The last line follows from the fact that $\actionsalt$ doesn't change the bids of winners under $\actions$, and for those agents, $\actionagent\geq\threshpt{\actionothers}$.
\end{proof}

An interpretation of this result is that the pay-your-bid greedy mechanism's welfare loss from incentives is limited to the multiplicative $\tfrac{e}{e-1}$ factor that appears in value covering. As a corollary, we obtain:

\begin{corollary}
The welfare of the pay-your-bid greedy combinatorial auction is a $\sqrt{\numitems}\tfrac{e}{e-1}$-approximation to that of any other mechanism.
\end{corollary}

Lemma~\ref{lem:rctorcr} implies revenue covering with reserves. We therefore have:

\begin{corollary}
With monopoly reserves and regular bidders, the revenue of the pay-your-bid greedy combinatorial auction is a $(\sqrt{\numitems}+1)\tfrac{e}{e-1}$-approximation to that of any other mechanism.
\end{corollary}




==> beyondpayyourbid_firstpricematroid.tex <==

\subsection{First Price Matroid Auctions}
\label{sec:fpamatroid}
In the single-item setting, both the revenue and the losers' threshold bids were the bid of the unique winner. In matroid settings, multiple winners complicates this relationship. Using standard matroid properties, we show how to untangle the relationship between threshold bids and winners' payments for the winner-pays-bid mechanism which allocates the bid-maximizing basis. We get, as corollaries, approximation guarantees identical to those achieved in the single-item case. In particular, we derive:

\begin{lemma}
\label{lem:pybrevcover}
The winner-pays-bid mechanism is 1-revenue covered in any matroid feasibility environment with any reserves.
\end{lemma}

\begin{corollary}\label{thm:welmat}
The welfare of the winner-pays-bid highest-basis-wins matroid auction is an $e/(e-1)$-approximation to that of any other mechanism.
\end{corollary}

\begin{corollary}\label{thm:revmat}
For the winner-pays-bid matroid auction with monopoly reserves and regular bidders, the revenue of any BNE is a $2e/(e-1)$-approximation to that of any other mechanism.
\end{corollary} 


We first develop the matroid-specific tools we need to relate bids (and therefore revenue) to the thresholds agents see. To do so, we use a property related to a result from \citet{T03} for VCG in matroid environments.
%is this just pointwise revenue covering?
%Hm. Yep.
\begin{lemma}
\label{lem:bidsvsthresholds}
Let $\bidalloc(\cdot)$ be the allocation rule which serves the bid-maximizing set of agents in a matroid environment. For any action profile $\actions$ and feasible allocation $\allocalt$:
\begin{equation} \label{eq:bidptwisecovred}
\sum\nolimits_\agent \actionagent\bidallocagent(\actions) \geq \sum\nolimits_\agent \threshpt{\actionothers}\allocaltagent.
\end{equation}
\end{lemma}

The proof is based on the following matroid property:

\begin{lemma}[Replacement Property]
\label{lem:rep}
Let $S_1$ and $S_2$ be independent sets of size $k$ in a matroid $\mathcal M$. Then there is a bijective function $\pi:S_2\setminus S_1\rightarrow S_1\setminus S_2$ such that, for every $\agent\in S_2\setminus S_1$, the set $(S_1\setminus\{\pi(i)\})\cup\{\agent\}$ is independent in $\mathcal M$.
\end{lemma}

\begin{proof}[\NOTEC{Proof} of Lemma~\ref{lem:bidsvsthresholds}]
Because subsets of feasible allocations are feasible, threshold bids are nonnegative, so we only need consider allocations $\allocalt$ which are bases. Let $\set$ and $\setalt$ be sets served by $\alloc$ and $\allocalt$, respectively. Since bids are nonnegative, it follows that $\set$ and $\setalt$ are the same size. By Lemma~\ref{lem:rep}, there exists a bijection $\pi$ from $\setalt\setminus\set$ to $\set\setminus\setalt$ with the replacement property in the lemma. For each $\agent\in\setalt\setminus S$, $\strategy_{\pi(\agent)}(\val_{\pi(\agent)})\geq \threshpt{\valothers}$, as if $\agent$ bids above $\strategy_{f(\agent)}$, then $(\set\setminus\{\pi(\agent)\})\cup\{\agent\}$ would be optimal and therefore $\agent$ would be allocated in BNE. For each $\agent\in\setalt\cap\set$, $\agent$ was served in $x(\val)$, it must be that $\stratagent(\valagent)\geq\threshpt{\valothers}$. The result follows by summing over $\agent$.
\end{proof}

Note that Lemma~\ref{lem:bidsvsthresholds} applies to any auction in a matroid environment where agents submit bids, and the mechanism selects a basis maximizing the sum of selected bids. We will make use of this lemma once more when discussing all-pay auctions, in Section~\ref{sec:allpay}.

Having established a relationship between threshold bids and bids of the winners, proving revenue covering is simply a matter of taking expectations.

\begin{lemma}
\label{lem:matrc}
The first-price matroid auction is 1-revenue covered.
\end{lemma}

\begin{proof}
Consider some alternate allocation $\allocalt$ and bid distribution $\actionsdist$. By the definition of winner-pays-bid mechanisms and Lemma~\ref{lem:bidsvsthresholds},
\begin{equation}
\rev(\mech,\actionsdist) =\expect[\actions]{\sum\nolimits_\agent \actionagent\bidallocagent(\actions)}\geq\expect[\actions]{\sum\nolimits_\agent \threshpt{\actionothers}\allocaltagent}
=\sum\nolimits_\agent \expect[\actions]{\threshpt{\actionothers}}\allocaltagent.\notag
\end{equation}
The result follows from the observation that $\expect[\actions]{\threshpt{\actionothers}}=\threshexpected{0}{1}$.
\end{proof}

Having proven revenue covering, Corollary~\ref{thm:welmat} follows from Theorem~\ref{thm:pybwelf}. Lemma~\ref{lem:rctorcr} implies revenue covering with reserves, which combine with Theorem~\ref{thm:pybrev} to prove Corollary~\ref{thm:revmat}.

==> framework.tex <==
\section{Framework}
\label{sec:revenuecovering}


In equilibria of the single-item first-price auction, we observed that agents with low expected utility had high expected threshold bids. Because high thresholds were connected to high payments, we could conclude that the first price auction is both approximately welfare- and revenue-optimal. The goal for this section is to build up a framework for making this same argument for mechanisms with different payment semantics, such as all-pay auctions. In particular, we seek to prove results about behavior in Bayes-Nash equilibrium while \emph{ignoring} the particular payment semantics of each auction. We begin by defining \emph{equivalent bids}, which allow us to reduce the optimization problem a bidder faces in any auction to the problem faced in a first-price auction. This will allow us to reduce much of the analysis of general auctions for single-dimensional agents to the single-item first-price auction analysis of Section~\ref{sec:easy}.

\subsection{Equivalent Bids}
Utility-maximizing agents must balance two goals: getting allocated frequently, and getting allocated cheaply. In a first-price auction, agents bid to explicitly specify the tradeoff they are willing to make: their bid is the price they pay per unit of allocation. In general mechanisms, for any agent $\agent$ and any action $\actionagent$, define the \emph{equivalent bid} for an action $\actionagent$ to be $\equivbidact{\actionagent}=\bidpaymentagent(\actionagent)/\bidallocagent(\actionagent)$; this can be thought of as the price per unit of allocation for that action. For first-price auctions, this is exactly the bid. For mechanisms with different payment semantics, $\equivbidact{\actionagent}$ can still be thought of as an equivalent first-price bid for action $\actionagent$.

\paragraph{Equivalent Threshold Bid.}
In proving Theorem~\ref{thm:fpawelfare}, we noted that $\bid$ is the minimum payment necessary to get the allocation probability $\bidallocagent(\bid)$. We used this property to bound the distribution of other agents' bids. For auctions where this relationship is less clear, we think of agents partitioning the actions in their choice set by interim allocation probability, then for each probability consider only the cheapest such action in terms of price per unit of allocation. For each allocation probability $\allocdev$, let $\effaction(\allocdev)$ be that cheapest action and let the \emph{equivalent threshold bid} $\ppu(\allocdev) = \equivbidact{\effaction(\allocdev)}$ be the equivalent bid of the cheapest action. Formally, $\ppu(\allocdev)= \min_{\actionagent:\bidallocagent(\actionagent)\geq \allocdev} \equivbidact{\actionagent}$, with $\effaction(\allocdev)$ the $\arg \min$. Note that $\ppu(\allocdev)$ depends on $\strat$; for notational convenience, we suppress the strategy profile as an argument. 

\paragraph{Cumulative Equivalent Threshold Bid.}
We can now use $\ppu(\allocdev)$ to track the expense an agent faces from increasing their allocation. Specifically, assume an agent is playing some action $\actionagent$ and seeks to increase their allocation probability to $\alloclevel$. The barrier to $\agent$ doing so is the set of equivalent threshold bids in $[\bidallocagent(\actionagent),\alloclevel]$. We can use this notion to measure $\agent$'s expense for additional allocation.  Define the \emph{cumulative equivalent threshold bid} as
$\threshexpected{\bidallocagent(\actionagent)}{\alloclevel}=\int_{\bidallocagent(\actionagent)}^{\alloclevel}\ppu(\allocdev)\,d\allocdev.$ If $\alloclevel\leq\bidallocagent(\actionagent)$, then define $\threshexpected{\bidallocagent(\actionagent)}{\alloclevel}=0$. This quantity will function identically to its counterpart in Section~\ref{sec:easy}, trading off against $\agent$'s surplus as in Lemma~\ref{lem:covering}, and translating into revenue as in Lemma~\ref{lem:monoprevapx}. Note that because $\ppu(\allocdev)$ is nondecreasing in $\allocdev$, $\threshexpected{\bidallocagent(\actionagent)}{\alloclevel}$ is convex in $\alloclevel$. 

\subsection{Covering Conditions and the Price of Anarchy}
\label{sec:frameworkpoa}
We now use equivalent bids and thresholds in place of first-price bids and thresholds to develop general analogues of the value and revenue covering conditions of Section~\ref{sec:easy}. 

\begin{lemma}[Value Covering]
\label{lem:vc}
Consider a mechanism $\mech$ in BNE with induced allocation and payment rules $(\alloc,\payment)$, and an agent $\agent$ with value $\valagent$. For any $\alloclevel\in[0,1]$,
\begin{equation}
\label{eq:vcl}
\valagent\allocagent(\valagent)+\threshexpected{\allocagent(\valagent)}{\alloclevel}\geq\tfrac{e-1}{e}\valagent\alloclevel.
\end{equation}
\end{lemma}

 The proof can now be done by reduction to the single-item first-price auction (Lemma~\ref{lem:covering}) because bidders now face effectively the same optimization problem as in a single-item first-price auction. The proof is \IFECELSE{left to the full version of the paper}{included in Appendix~\ref{sec:appframework}}. 
 
 To prove an approximation result for welfare or revenue, the \emph{only} mechanism-specific detail which remains is specifying the relationship between $\expthresholdagent$ and the mechanism's revenue. Intuitively, we saw in Section~\ref{sec:easy} that if there is a relationship between revenue and the difficulty an agent faces in increasing their allocation once they have chosen to participate in the mechanism, then value covering allows us to show a welfare bound. To make this relationship concrete, we extend the definition of Lemma~\ref{lem:monoprevapx}.

\begin{definition}[Revenue Covering]
\label{def:rc}
A mechanism $\mech$ is \emph{$\revpar$-revenue covered} if for any (implicit) strategy profile $\strat$, feasible allocation $\allocalt$, and action profile $\actions$,
\begin{equation*}
\revpar \rev(\mech)\geq\sum\nolimits_\agent \threshexpected{\bidallocagent(\actionagent)}{\allocaltagent}.
\end{equation*}
\end{definition}

Note that Definition~\ref{def:rc} makes no mention of BNE. It must hold for any strategy profile. This is a stronger condition than Lemma~\ref{lem:monoprevapx}, as it is not restricted to bidders with values above a set of reserves or bidders playing only participatory strategies. 

As we already saw, revenue covering has a number of important consequences. First is a welfare bound.

\begin{theorem}
\label{thm:poa}
If a mechanism is $\revpar$-revenue covered, then in any BNE it is a $(1+\mu)\frac{e}{e-1}-$approximation to the welfare of the optimal mechanism.
\end{theorem}

\begin{proof}
Let $\allocopt$ be the welfare-optimal allocation rule. For any value profile $\val$, Lemma~\ref{lem:vc} with $\alloclevel=\allocoptagent(\val)$ yields that for each $\alloc$,
\begin{equation*}
\valagent\allocagent(\valagent)+\threshexpected{\allocagent(\valagent)}{\allocoptagent(\val)}
	\geq\tfrac{e-1}{e}\valagent\allocoptagent(\val).
\end{equation*}
\noindent
Summing over agents and using revenue covering gives
$\sum\nolimits_\agent \valagent \allocagent(\valagent) + \revpar \rev(\mech)
\geq \tfrac{e-1}{e} \sum\nolimits_\agent \valagent \allocoptagent(\val).
$  Taking expectation with respect to $\val$ and using $\WEL(\mech)\geq \rev(\mech)$, we get 
\begin{equation}
(1+\revpar)\frac{e}{e-1} \rev(\mech)\geq \frac{e}{e-1}\WEL(\OPTmech).
\end{equation} 
\end{proof}

%\subsection{Connection to Smoothness}
%\citet{ST13} give a method for proving price of anarchy bounds for mechanisms using deviation strategies and the observation that the utility from these deviation strategies lower bounds agents' equilibrium utilities. By choosing deviations that relate to the payments of the mechanism, one can combine utilities and payments to get welfare bounds. On a high level, this approach strongly mirrors ours. Lemma~\ref{lem:vc} can be rearranged into a lower-bound on surplus. We then relate the lower bound to the mechanism's revenue using Definition~\ref{def:rc}.

%The connection between value covering and the deviation bid is especially close. Much of the theoretical machinery in the paper is designed to draw analogies between general mechanisms and those with first-price payment sematics. We can exploit this analogy and use the deviation bid for the first-price auction without reserves from \citep{ST13} to prove Lemma~\ref{lem:vc} in a second way. We give a sketch of the proof technique, but omit details which can be found in \citep{ST13}.

%The Bayesian deviation given in \citep{ST13} is for each agent $\agent$ to mix between drawing a bid from a particular distribution $\sd$ which depends on her value (with probability $\alloclevel$) and bidding zero (with probability $1-\alloclevel$). This yields expected utility at least $\valagent\alloclevel e/(e-1)-\expect[\valothers]{\maxbidothers(\valothers)}$, where $\maxbidothers$ is the highest competing bid from other agents. In a general mechanism, the analogous deviation is to mix between drawing an equivalent bid from $\sd$ and playing the best action corresponding to this bid (with probability $\alloclevel$) and bidding to get expected utility zero (with probability $1-\alloclevel$). Note that such a deviation requires knowledge of other agents' equilibrium strategies, but can be defined for the equilibrium of any mechanism. The expected utility from this deviation is at least $\valagent\alloclevel e/(e-1)-\threshexpected{0}{1}$. Note that $\expect[\valothers]{\maxbidothers(\valothers)}=\threshexpected{0}{1}$ in the first-price auction with no reserves.

\subsection{Revenue Covering With Reserves}
\label{sec:RRC}
%Smoothness approaches hinge on proving price of anarchy bounds in a restricted way. The restricted proofs imply extensions to broader environments. Our framework operates in this spirit, and to obtain a reserves extension, we impose similar restrictions.

%We will make use of two restrictions to revenue covering in order to extend. First, revenue covering can apply for only a certain set of agents --- that is, the revenue of a mechanism covers the thresholds of only a certain set of agents. Second, we can restrict

%\paragraph{Restrictions for Reserves}
Not all agents need their thresholds covered for a welfare and revenue approximation result. For instance, in Section~\ref{sec:easy}, we considered the first-price auction with monopoly reserves. Bidders with values below their reserve experience a threshold created by the reserve of the auction which does not translate into revenue. We showed instead that revenue covers the thresholds for bidders with values (and hence equilibrium bids) above their reserves, which was sufficient for approximation results because the optimal auction served no bidder with value below their reserve. 

%We now formalize this notion of revenue covering restricted to certain agents. We will specify a restriction using a mapping $\filter$ from value profiles to allowed agents, specifying the agents whose thresholds will be covered. In the case of individual reserves $\reserves=(r_1,\ldots,r_n)$, $\filter(\vals)=\{\agent\ |\ \valagent\geq \reserveagent\}$, the set of all agents with values above their individual thresholds. 

%how to introduce this the right way??
For the actions of such agents to be revenue covered, we do need bidders with values above their reserve to bid at least the reserve, just as in Section~\ref{sec:easy}. Given a strategy profile $\strat$ and value profile $\val$, define an action $\actionagent$ to be participatory for $\strat$ and $\val$ if the equivalent bid $\equivbidact{\actionagent}\leq v_i$ and either $\bidallocagent(\actionagent)>0$  or there is no alternate action $a_i'$ that gives $i$ strictly positive utility. Note that participatory is a much weaker assumption than equilibrium or best-response; it only specifies that bidders play some action that gives positive allocation if there is such an (IR) action. Thus in BNE, all bidders will play participatory actions.

%(For example, consider a first price auction where all bidders other than $\agent$ have bid supports which are bounded away from 0. Small positive bids for $\agent$ yield no allocation, but $\agent$ is indifferent between these bids and withdrawing, so we shouldn't distinguish between these actions.)

\begin{definition}[Revenue Covering with Reserves]
\label{def:restricted2}
\label{def:revcoverabove}
A mechanism $\mech$ is $\revpar$-revenue covered with reserves $\reserves=(\reserve_1, \ldots,\reserve_n)$ if for any (implicit) strategy profile $\strat$, value profile $\val$, feasible allocation $\allocalt$, and participatory action profile $\actions$,
\begin{equation*}
\revpar\rev(\mech)\geq\sum\nolimits_{i : \valagent> \reservei} \threshexpected{\bidallocagent(\actionagent)}{\allocaltagent}.
\end{equation*}
\end{definition}

Note that revenue covering above reserves is a weaker condition than general revenue covering, and is not relying on any specific property of the mechanism, like whether it does or does not have reserves. For instance, the first price auction with no reserves will satisfy revenue covering with any reserves.

\begin{theorem}
\label{thm:reswel}
If a mechanism $\mech$ is $\revpar$-revenue covered with reserves $\reserves=(\reserve_1, \ldots,\reserve_n)$, then the welfare of $\mech$ is a $(1+\revpar)e/(e-1)$-approximation to the welfare of the optimal mechanism which only serves agents with value $\valagent\geq \reservei$.
\end{theorem}
\begin{proof}
Let $\allocopt$ be the welfare-optimal allocation rule, and consider some value profile $\val$. Lemma~\ref{lem:vc} with $\alloclevel=\allocoptagent(\val)$ yields that for each $\alloc$ and value $\valagent$,
\begin{equation}
\valagent\allocagent(\valagent)+\threshexpected{\allocagent(\valagent)}{\allocoptagent(\val)}
	\geq\tfrac{e-1}{e}\valagent\allocoptagent(\val).\notag
\end{equation}

As all bidders in BNE play participatory actions, summing over all agents with values above reserves and using revenue covering yields:
\begin{equation}
\sum\nolimits_{\agent:\valagent > \reservei} \valagent \allocagent(\valagent) + \revpar \rev(\mech)
\geq \tfrac{e-1}{e} \sum\nolimits_{\agent:\valagent > \reservei} \valagent \allocoptagent(\val). \notag
\end{equation}

Taking expectation with respect to $\val$, noting that $\allocopt$ only serves agents with $\valagent\geq \reservei$ and agents have value $\reservei$ with probability $0$, we get $ \WEL(\mech)+\revpar \rev(\mech)\geq\frac{e-1}{e}\WEL(\OPTmech)$; hence $ (1+\revpar)\frac{e}{e-1} \rev(\mech)\geq\frac{e}{e-1}\WEL(\OPTmech)$.
\end{proof}


%DH - Commenting out for now - can we get away with not even talking about it?

%\paragraph{Covering-Preserving Reserves}
%For many auctions, it is possible to add reserves to a revenue covered mechanism and preserve revenue covering restricted to bidders with values above the implemented reserves. As a result, the BNE welfare of the reserves mechanism approximates the welfare of the optimal mechanism that serves only those agents. In \IFECELSE{the appendices of the full version of this paper}{Appendix~\ref{sec:appres}}, we provide a general set of conditions under which reserves preserve revenue covering in this manner. These conditions hold, for example, in first-price matroid and position auctions, as well as under simultaneous composition. These mechanisms with reserves consequently meet the conditions of Lemma~\ref{thm:reswel}, yielding a welfare approximation, and as we show in the next section, a revenue approximation.

==> revenuecovering.tex <==
\section{Revenue Covering}
\label{sec:welfare}
We have now shown that revenue-covering is a sufficient condition for a number of welfare and revenue approximation results:
\begin{itemize}
\item If $\mech$ is $\revpar$-revenue covered, the welfare of $\mech$ is a $(1+\mu)\frac{e}{e-1}-$approximation to the optimal welfare. (Theorem~\ref{thm:poa} in Section~\ref{sec:frameworkpoa}) 
\item If $\mech$ implements monopoly reserves $\reserves^*$ and is $\revpar$-revenue covered with $\reserves^*$, the revenue of $\mech$ is a $(1+\mu)\frac{e}{e-1}-$approximation to the optimal revenue. (Lemma~\ref{lem:monopreserves} in Section~\ref{sec:reserveprices})
\item If $\mech$ is $\revpar$-revenue covered and implements $k-$duplicates, the revenue of $\mech$ is a $(\frac{k}{k-1} + \revpar )\frac{e}{e-1}$-approximation to the optimal revenue. (Corollary~\ref{cor:kbiddersrev} in Section~\ref{sec:duplicates})
\end{itemize}

In this section, we show that many auctions beyond the single-item, first-price auction are revenue covered, and thus get new welfare and revenue approximation results for each. %Missing proofs are included in \IFECELSE{the appendices of the full version of this paper}{Appendix~\ref{sec:apprevcovering}}.

\subsection{First Price Matroid Auctions}
In our discussion of the single-item case (Section~\ref{sec:easy}), we saw that when an agent has trouble getting allocated in a first price auction (that is, the cumulative additional threshold $\expthresholdagent$ is high), it is because other agents submit high bids. These competing bids translate into revenue, implying that the first-price auction is 1-revenue covered. With one extra step, this reasoning extends to first-price auctions where the feasible allocations form a matroid. An agent's threshold bid does not precisely correspond to a competing bid, but matroid properties provide a sufficiently close analog, implying revenue covering. Combining with Theorem~\ref{thm:poa} and Lemma~\ref{lem:monopreserves} respectively imply welfare and revenue approximations of $2e/(e-1)$ with reserves. If the auction implements $k$-duplicates, which happens in the single-item setting when at least $k$ bidders have values drawn from each distribution, then by Corollary~\ref{cor:kbiddersrev} it is a $\frac{k}{k-1}\frac{2e}{e-1}$ approximation to the revenue optimal mechanism.

\begin{lemma}
\label{lem:pybrevcover}
The first-price auction is 1-revenue covered in any matroid feasibility environment.
\end{lemma}

The proof is included in Appendix~\ref{sec:apprevcovering}.




\subsection{Position Auctions}
In first-price position auctions (a.k.a., the generalized first-price auction, GFP), arguments similar to those in the matroid case yield analogous welfare and revenue guarantees.

Formally, a position auction is an auction in which agents can be allocated one of $m$ positions; each of which is valued by an agent at $\alpha_j \valagent$. In advertising auctions, these are slots on a webpage to fill where lower slots receive fewer clicks. The positions are ordered such that $\{\alpha_j\}$ is decreasing in $j$ (hence slot 1 is best).

In GFP, agents submit bids $\bid_i$, and positions are allocated in order of bid. Each agent pays their bid scaled by the quality of the slot:  $\alpha_j \bid_i$. Equivalently, they pay their bid when they are served, which occurs with probability $\alpha_j$ for position $j$.

While the correspondence between bids and threshold bids is not as immediate in GFP as in the single-item, first-price auction, GFP satisfies a notion of pointwise revenue covering, or revenue covering when other players are playing fixed actions that we use to show that it satisfies general revenue covering. The proof is included in \ref{sec:apprevcovering}. By Lemma~\ref{lem:fpaaddingreserves}, adding reserves preserves revenue covering above the reserves and so Theorem~\ref{thm:poa} and Lemma~\ref{lem:monopreserves} respectively imply welfare and revenue approximations of $2e/(e-1)$ with reserves. 

\begin{theorem}\label{thm:gfp-covered}
The generalized first price (GFP) auction is $1$-revenue covered.
\end{theorem}


\subsection{All-Pay Auctions}
Revenue-covering is not limited to first-price semantics: the all-pay is also revenue covered, with $\mu=2$. The relationship between revenue and thresholds in an all-pay auction is more indirect than for the first price auction. In a first-price auction, if a bidder must bid $\$10$ to attain a $80\%$ probability of winning, it must be because the highest bid from other bidders is greater than $\$10$ $80\%$ of the time. In an all-pay auction however, the bidder would have to always pay $\$10$ instead. Recall that the equivalent bid of an action is the price per unit of allocation, so the equivalent bid of the $\$10$ all-pay bid giving allocation of $80\%$ is $\$10/80\%=\$12.50$ which is more than the competing bids that induced the threshold. 

As the allocation probability from an all-pay bid approaches $1$, the equivalent bid approaches the all-pay bid, and so such bids are almost revenue-covered. For small probabilities of allocation however, the all-pay bid and equivalent bid may be very far apart. The proof uses the monotonicity of the allocation rule to show that the threshold from bids with high probabilities of allocation outweighs the threshold from bids with low probabilities of allocation, giving a bound for the cumulative additional threshold of at most twice the revenue of the auction.

Combining with Theorem~\ref{thm:poa} gives a welfare bound of $3e/(e-1)$, weaker than the bound of $2$ in \citet{ST13}. For revenue, it is not feasible to add reserves to an all-pay auction, but the all-pay auction with at least $k$-bidders from each distribution satisfies $k$-duplicates, and thus by Corollary~\ref{cor:kbiddersrev} the revenue of the all-pay auction with at least $2$ bidders with values from each distribution is a $4e/(e-1)$-approximation to the revenue of the optimal auction.


\begin{lemma}
\label{lem:aprc}
The all-pay matroid auction is 2-revenue covered.
\end{lemma}
We include the proof here for the single-item case; the generalization to matroids is included in Appendix~\ref{sec:apprevcovering}.
\begin{proof}[Proof (single-item).]
We first translate revenue to threshold bids. In expectation, these thresholds 2-approximate the equivalent threshold bids. Combining the two arguments yields the result.

Let $\strat$ be an arbitrary strategy profile, and $\allocalt$ an alternate allocation. First, for any bidder $\agent$, let $\critbid{\valothers}$ be the threshold (all-pay) bid for $\agent$ in realized value profile $\valothers$ under $\strat$. Since the threshold bid corresponds to some other agent's bid, and agents pay their bids regardless of allocation, $\rev(\mech)\geq \expect[\valothers]{\critbid{\valothers}}\geq\expect[\valothers]{\critbid{\valothers}}\allocaltagent.$

To relate threshold bids to equivalent thresholds, let $\actionagent(\allocdev)$ be the $\allocdev$-quantile of $\agent$'s competing bids. That is, $\actionagent(\allocdev)=\argmin_{\actionagent}$ $\bidpaymentagent(\actionagent)$ subject to $\bidallocagent(\actionagent)\geq\allocdev$. By the definition of $\ppu$,
\begin{equation}
\frac{\bidpaymentagent(\actionagent(\allocdev))}{\bidallocagent(\actionagent(\allocdev))}\geq\ppu(\allocdev).\notag
\end{equation}
Rearranging and noting that in an all-pay auction, $\bidpaymentagent(\actionagent(\allocdev))=\actionagent(\allocdev)$, we obtain
\begin{equation}
\label{eq:bvtbound}
\actionagent(\allocdev)\geq\ppu(\allocdev)\bidallocagent(\actionagent(\allocdev))\geq\ppu(\allocdev)\allocdev.
\end{equation}

This yields the following sequence of inequalities:
\begin{equation}
\label{eq:bidtothresh}
\expect[\valothers]{\critbid{\valothers}}=\int_0^1 \actionagent(\allocdev)\, d\allocdev \geq
\int_0^1\ppu(\allocdev)\allocdev\,d\allocdev\geq
 \frac{1}{2} \int_0^1 \ppu(\allocdev)\, d\allocdev=\threshexpected{0}{1},
\end{equation}
where the first equality follows from noting that expected value can be computed by integrating over quantiles, the first inequality from equation \eqref{eq:bvtbound}, and the second inequality from the fact that $\ppu$ is an increasing function and Chebyshev's sum inequality. Finally, since $\allocalt$ is feasible, $\sum\nolimits_\agent \allocaltagent\leq 1$. We can combine this with (\ref{eq:bidtothresh})  to get
\begin{equation}
2\rev(\mech)\geq\sum\nolimits_\agent \threshexpected{0}{1}\allocaltagent.
\end{equation}

By the convexity of $\expthresholdagent$, $\threshexpected{0}{1}\allocaltagent\geq\threshexpected{0}{\allocaltagent}$. Since $\threshexpected{0}{\allocaltagent}\geq\threshexpected{\bidallocagent(\actionagent)}{\allocaltagent}$, we conclude that the all-pay auction is 2-revenue covered.
\end{proof}


\subsection{The Second-Price Auction}
\label{sec:spa}
Not all mechanisms are revenue covered. One such mechanism that lacks a direct relationship between thresholds and revenues is the second-price auction. In the second-price auction, agents submit sealed bids, the highest bidder wins and is charged the second-highest bid. Consider a two-agent setting where bidders have deterministic values $v_1=1$ and $v_2=\epsilon$. Assume agent 1 bids 1 and agent 2 bids $\epsilon$. The revenue is $\epsilon$, but $T_2[0,1]$ is 1, so the second-price auction cannot be revenue covered.

==> simultaneouscomposition.tex <==
\section{Extension: Simultaneous Composition}
\label{sec:simul}
In this section we prove that if a set of mechanisms satisfy revenue covering when operated in isolation, then they satisfy revenue covering when many instances of the mechanisms are simultaneously being run if agents are unit-demand and single-valued across outcomes of the mechanisms. We formally define simultaneous composition for single-dimensional agents as follows:

\begin{definition}
Let mechanisms $\mech_1,\ldots,\mech_m$ have allocation and payment rules $(\allocitem,\paymentitem)$ and individual action spaces spaces $A_\agent^1,\ldots,A_\agent^m$ for each agent $\agent$. The \emph{simultaneous composition} of $\mech_1,\ldots,\mech_m$ is defined to have:
\begin{itemize}
\item Action space $\prod_\mitem A_\agent^\mitem$ for each agent. That is, each agent participates in the global mechanism by participating in each composed mechanism individually. 
\item Allocation rule $\bidallocagent(\actions)=\left [\bidallocagent^1(\actions^1),\ldots,\bidallocagent^m(\actions^m)\right].$ In other words, the mechanism gives each agent their allocated bundle from each mechanism.
\item Payment rule $\bidpaymentagent(\actions)=\sum_\mitem \bidpaymentagentitem(\actionsitem)$. That is, agents make payments to every composed mechanism.
\end{itemize}
\end{definition}

We assume agent utilities are \emph{unit demand} and \emph{single-valued} over the outcomes of the mechanisms. Agent utilities are then of the form $\valagent \cdot(\max_{\mitem\in\wantsagent}\bidallocagentitem(\actions))-\bidpaymentagent(\actions)$. The \emph{induced single-dimensional allocation rule} is $\simallocagent(\actions)=\max_{\mitem\in\wantsagent}\bidallocagentitem(\actions)$; it serves the same role in our framework as the allocation rule of a single, uncomposed mechanism. We define $\thresholdagent$, $\expthresholdagent$, and revenue covering with respect to $\simallocagent$ for mechanisms defined as in previous sections.

The main theorem of this section is that the simultaneous composition of a number of mechanisms that satisfy the same notion of revenue covering (no reserves, or above the same individual reserves) remains revenue covered in the same manner.

\begin{lemma}
\label{lem:seq}
Let $\mech$ be the simultaneous composition of $\revpar$-revenue covered (with reserves $\reserves$) mechanisms $\mech_1, \ldots \mech_m$ with unit-demand, single-valued agents; then $\mech$ is $\revpar$-revenue covered (with reserves $\reserves$).
\end{lemma}

The proof is included in \IFECELSE{the full version of this paper}{Appendix~\ref{sec:appsim}}. Combining Lemma~\ref{lem:seq} with Theorem~\ref{thm:poa} and Lemma~\ref{lem:monopreserves} immediate yields welfare and revenue results, for instance:

\begin{corollary}
Let $\mech$ be the simultaneous composition of $k$ first-price auctions with monopoly reserves $\reserves^*$, matroid feasibility constraints, and unit-demand, single-valued agents with regularly distributed valuations. Then, the revenue of $\mech$ is a $\frac{2e}{e-1}-$approximation to the revenue of the optimal global mechanism. 
\end{corollary}

%Recall that restricted revenue covering implies revenue covering in the unrestricted sense. This, in turn, immediately yields a welfare result. We prove an analogous result for revenue covering with restrictions to handle reserves in \IFECELSE{the full version of this paper}{Appendix~\ref{sec:appsim}}, and therefore derive composition composition (and therefore welfare and revenue results) for composed mechanisms with reserves.

%\subsection{Reserves in Simultaneous Composition}
%To implement reserves $\reserves$ in the simultaneous composition of $m$ single-item first-price auctions $\mech$, define the reserves mechanism $\mechr$ by discardin the bids of any agent $\agent$ who bids below $\reserveagent$ in any of the composed mechanisms. The reserves mechanism therefore gives those agents zero allocation and payments.

%These reserves are covering-preserving, and respect $\actspacealt$ as defined above. We verify each part of Definition~\ref{def:res} separately.
%\begin{enumerate}
%\item In BNE, agents would rather withdraw than overbid in any auction. For agents with $\valagent\leq\reserveagent$, overbidding is the only way to get allocated, so no such agent is allocated in BNE.
%\item To compute $\strat$ from $\stratres$, have any agent bidding below their reserves in any auction withdraw from the global mechanism instead.
%\begin{enumerate}
%\item The payments and allocations between $\stratres$ and $\strat$ are identical, as the reserves mechanism forces overbidding agents to withdraw, but is otherwise identical to the version without reserves.
%\item In the composed first price auction without reserves, $\allocmin=0$, and $\allocrmin$ cannot be negative. Specifically, $\allocrmin$ is the minimum over all items of the probability that all other agents bid below $\reserveagent$ for that item in $\stratres$.
%\item Let $\allocdev\geq\allocrmin$. To get allocated in $\mech$ with probability at least $\allocdev$ using only actions in $\actspaceagentalt$, $\agent$ must bid at least $\reserveagent$ on some item. But such a bid is also an option for $\agent$ in $\mechr$, the equivalent bid for that action in $\mechr$ under $\stratres$ is at most its equivalent bid in $\mech$ under $\strat$. It follows that $\thresholdragent(\allocdev)\leq\thresholdagentrest(\allocdev)$,
%\end{enumerate}
%\end{enumerate}

%As a consequence of Lemma~\ref{lem:monopreserves}, introducing monopoly reserves to the simultaneous composition of single-item first-price auctions in the way described yields a mechanism which $2e/(e-1)$-approximates the revenue of the optimal mechanism for agents with regular value distributions.
